Exploring the Impact of COVID-19 Lockdown on Social Roles and Emotions while Working from Home

In the opening months of 2020, COVID-19 changed the way for which people work, forcing more people to work from home. This research investigates the impact of COVID-19 on five researchers' work and private roles, happiness, and mobile and desktop activity patterns. Desktop and smartphone application usage were gathered before and during COVID-19. Individuals' roles and happiness were captured through experience sampling. Our analysis show that researchers tend to work more during COVID-19 resulting an imbalance of work and private roles. We also found that as working styles and patterns as well as individual behaviour changed, reported valence distribution was less varied in the later weeks of the pandemic when compared to the start. This shows a resilient adaptation to the disruption caused by the pandemic.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> Sections/Experiments_pre.tex <==

After clustering, and choosing the optimal number of clusters using silhouette analysis. We found that silhouette analysis showed that 13 clusters was the optimal size. These clusters corresponded to the 12 different categories chosen + 1 cluster filled with segments with no activity at all. This was determined by the distribution of the average segment in a cluster. Each cluster had one category that was prominent. Figure~\label{seg:12} shows segment 12 for which we named the "Developer Tools" cluster.

\begin{figure}[ht] \label{fig:seg12}
    \centering
    \includegraphics[width=\linewidth]{images/AverageSegmentBar/Segment-12.png}
    \caption{Bar chart showing average distribution for segments clustered into the "Developer Tools" cluster}
    \Description{Bar chart with Computer Tools as the largest value, and Utilities and Browsers coming a little higher after than}
\end{figure}

A dendrogram was then plotted to show the relationship between all the different clusters.
The dendrogram shows that the Nothing cluster is maximally different from all other segments (as expected due to our modified cosine similarity, see section~\ref{appusageanalysis}) and that the Computer Tools is most similar to the Utilities cluster.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/Dendrogram/FullDendrogram.png}
    \caption{Dendrogram showing relationship between segments}
    \Description{A dendrogram showing the 13 different relationships. The segments show the null segment to be the least similar to the rest, and Developer Tools being commonly used alongside Utilities}
\end{figure}


==> Sections/Introduction_pre.tex <==
\section{Introduction}
% Ok, what's the scope of this study again?
% COVID-19's impact on: Happiness + the increase
In the opening months of 2020, the COVID-19 pandemic occurred. This changed the way that we lived our lives, encouraging more people to work from home. This has impacted the way that people work as well as their outlook on the world.

Although COVID-19 has had a large impact on the world, there has been little literature on its effects on the individual's productivity, happiness and work life balance. The challenge with researching this is that a large amount of specific data collected on this would have to been collected before COVID-19 for comparison.

This study capitalises on a large amount of information collected before the pandemic that was collected for a different study. This study therefore allows
a fair comparison between the lives of individuals before and after COVID-19 on a personal level.

This study looks into the effects of COVID-19 from two angles. Firstly, it contributes to the literature of the psychological effects of COVID-19 \cite{zhang_unprecedented_2020, li_impact_2020, losada-baltar_were_2020, kleinberg_measuring_2020} by looking into the effect that COVID-19 has had on the happiness and excitability of individuals before and during the virus.

This study also takes a look into how the individuals social roles were impacted before and after COVID-19. That is, how often an individual finds themselves in a private or work related role, or a combination of the two. 

We hypothesized that working from home would cause a significant increase in the amount of times the participants reported being in a "Work \& Private" role. We also hypothesized that COVID-19 would cause individuals to be less happy. We found neither of those hypothesis to be strongly supported.

\subsection{Research Questions}
In this paper, we attempt to answer the following questions:

\begin{enumerate}
    \item Did the introduction of COVID-19 correlate with a decrease in reported happiness individuals?
    \item Did the introduction of COVID-19 correlate with people reporting being in a more combined work and private role?
\end{enumerate}

\subsection{Research Challenges}
The main challenge with this research was with data collection. COVID-19 could not be anticipated and have the data controlled in such a way.

This problem was solved by utilising very detailed data collected for a different study before COVID-19, and recollecting the same data during the pandemic. This allowed for a comprehensive comparison between the behaviour of individuals before and after COVID-19.

The data was collected through an application installed on their computer or smartphone, which collected information as detailed in the Methods section.

\subsection{Proposed Contributions}
This paper aims to provide an insight as to how COVID-19 impacts personal lives, and contributes to the literature of the effect COVID had on individuals and what can be done to better understand individual behaviour in times of crisis. As well as showing how experience sampling can be used to measure the impact of pandemics and other crisis.


The rest of the paper is organized as follows. Section~\ref{sec:related} briefly introduces the related work. Section~\ref{sec:data} describes the data sets used in this paper and their collection methodology. The detailed methodologies for conducting each analysis are presented in Section~\ref{method}. Section~\ref{results} presents the outcome of the analysis. The limitations of this work and some discussions are presented in Section~\ref{dis}. Finally, this paper is concluded in Section~\ref{conclusion}.

==> Sections/Metodology_pre.tex <==


We then analysed the information collected on application usage to determine the similarity.

To find meaning in the segments found, we used agglomerative clustering. Agglomerative clustering is a technique for clustering data by linking the two closest elements in a set to each other, and then continuing to link other elements together until you are left with one set containing all elements.

Agglomerative clustering requires some distance metric to determine the distance between each segment. This poses an interesting problem as we are comparing segments with are multivariate time series.

Inspired from Sadri~\cite{sadri_information_2017}, who calculated the entropy of a multivariate time series by aggregating the result into a probability distribution representing how much of each channel (in our case, application) appeared in the segment before calculating the entropy of that distribution, we aggregated the probability distribution in the same way and used a modified cosine similarity to determine the distance between the two segments.

Our modified cosine similarity accounts for the possibility of having a distribution where no activity occurred to be a segment. As the cosine similarity between two segments where one or both segments has no activity is undefined. As our segments did include periods where no activity occurred, we redefined cosine similarity so that if one of the distributions was null but the other wasn't the distance from the distribution was maximum (1), but if they are both null, the distance between the distributions was 0.

We used average linkage in agglomerative clustering, meaning that the when comparing the distance between two clusters, the average of the distances between each element was used.

The output of agglomerative clustering is a hierarchy of elements. We can then choose the number of clusters that we want $n$, and get $n$ clusters which were linked together last during clustering.

To determine the most effective $n$, we used silhouette analysis.

==> Sections/Related_Work_pre.tex.tex <==
To exploit the impact of COVID-19 on personal level, this study conducts different type of analysis. It includes measuring the impacts of COVID-19 on a person's psychology, e.g. happiness and his social role. 

%\subsection{Experience Sampling}
%Experience sampling is the "representative sampling of immediate experiences in one’s natural environment"~\cite{beal_esm_2015}. It involves collecting detailed information  about the lives of participants for a brief period of time. This study is composed of two such periods of experience sampling.Experience sampling is designed to report the actual state of the participant as they go throughout their day, and it prevents memory biases that could be prevalent in this study if a more retrospective approach wa

==> images/Dataset_pre.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{rc}
       \toprule
       Category & Number of Apps \\
       \midrule
       Browser  & 7 \\
       Communication & 24 \\
       Developer Tools & 15  \\  
       Entertainment & 10 \\
       Game & 5 \\
       Media Viewing & 8 \\
       Reading & 6 \\
       Settings & 2 \\
       Tools & 26 \\
       Utilities & 23 \\
       Work Communication & 5 \\
       Writing & 8 \\ 
       \bottomrule
    \end{tabular}
    \caption{Categories chosen to summarise the application data}
    \label{tab:categories}
\end{table}
